Convex Optimization of Launch Vehicle Ascent Trajectory with Heat-Flux and Splash-Down Constraints

This paper presents a convex programming approach to the optimization of a multistage launch vehicle ascent trajectory, from the liftoff to the payload injection into the target orbit, taking into account multiple nonconvex constraints, such as the maximum heat flux after fairing jettisoning and the splash-down of the burned-out stages. Lossless and successive convexification are employed to convert the problem into a sequence of convex subproblems. Virtual controls and buffer zones are included to ensure the recursive feasibility of the process and a state-of-the-art method for updating the reference solution is implemented to filter out undesired phenomena that may hinder convergence. A hp pseudospectral discretization scheme is used to accurately capture the complex ascent and return dynamics with a limited computational effort. The convergence properties, computational efficiency, and robustness of the algorithm are discussed on the basis of numerical results. The ascent of the VEGA launch vehicle toward a polar orbit is used as case study to discuss the interaction between the heat flux and splash-down constraints. Finally, a sensitivity analysis of the launch vehicle carrying capacity to different splash-down locations is presented.

==> proof.tex <==

% \label{app:proof}

The proof that the optimal solution of $\mathcal{P}_R$ is the optimal solution also of problem $\mathcal{P}_A$ is here provided. 
Proposition~\ref{proposition:relaxation} is proved by contradiction, using the direct adjoint approach~\cite{hartl1995survey}. 
We introduce the Hamiltonian $H$:
\begin{equation}
    H = \bm{\lambda} \cdot \bm{f}(\bm{x}, \bm{u}, t) = \bm{\lambda}_{r} \cdot \bm{v} 
    + \bm{\lambda}_{v} \cdot \left(-\frac{\mu}{r^3} \bm{r} + \bm{u} 
    + \frac{T_b - D}{m} \bm{\hat{v}}_{\text{rel}} 
    + \frac{T_c}{m} \bm{\hat{r}}\right)
    + \lambda_m \left(-\dot{m}_e \right)
    \label{eq:hamiltonian}
\end{equation}
where $\bm{\lambda}(t) = \begin{bmatrix}
    \bm{\lambda}_{r}^T & \bm{\lambda}_{v}^T & \lambda_m
\end{bmatrix}^T$ is the costate vector, conveniently split in position, velocity, and mass subvectors. 
To take into account the path constraints, the Lagrangian $L$ is defined:
\begin{equation}
    L = H - \mu_Q (\dot{Q} - \dot{Q}_{\text{max}}) - \mu_u (u_x^2 + u_y^2 + u_z^2 - u_N^2) 
    \label{eq:lagrangian}
\end{equation}
where $\mu_u(t)$ and $\mu_Q(t)$ are the Lagrange multipliers associated with the constraints \eqref{eq:thrust_direction_cone_con} and \eqref{eq:heat_flux_nonlinear}, respectively.
The optimal solution
% $\{ \bm{x}^\star, \bm{u}^\star, t_f^\star \}$
must satisfy the complementary slack conditions:
\begin{align}
    \mu_Q \geq 0 &, \quad \mu_Q (\dot{Q} - \dot{Q}_{\text{max}}) = 0 \label{eq:complementary_condition_Q} \\
    \mu_u \geq 0 &, \quad \mu_u \left(u_x^2 + u_y^2 + u_z^2 - u_N^2\right) = 0 \label{eq:complementary_condition_u}
\end{align}
According to Pontryagin's minimum principle, the optimal control $\bm{u}^{\star}$ must be such that:
\begin{equation}
    \bm{u}^{\star} = \arg \min_{\bm{u} \in \mathcal{U}} H(\bm{x}^{\star}, \bm{u}, \bm{\lambda}, t)
\end{equation}
where $\mathcal{U}$ is the set of controls that satisfies Eq.~\eqref{eq:thrust_direction_cone_con}:
\begin{equation}
    \mathcal{U}(\bm{x}, t) = \left\{ \left(u_x, u_y, u_z \right) : u_x^2 + u_y^2 + u_z^2 \leq \left( \left(T_{\text{vac}} - p A_e\right) / m \right)^2 \right\}
\end{equation}
where $u_N$ was replaced with Eq.~\eqref{eq:u_N}.
The Karush–Kuhn–Tucker (KKT) condition for minimizing the Hamiltonian over $\bm{u} \in \mathcal{U}$ is:
\begin{equation}
    \frac{\partial L}{\partial \bm{u}} = \bm{\lambda}_{v} - 2 \mu_u \bm{u} = 0 \label{eq:KKT} 
\end{equation}

The costate equations are:
\begin{equation}
    \dot{\bm{\lambda}} = -\frac{\partial L}{\partial \bm{x}} = - \left[ \frac{\partial \bm{f}}{\partial \bm{x}} \right]^T \bm{\lambda} - \mu_Q \frac{\partial\dot{Q}}{\partial \bm{x}} - 2 \mu_u u_N \frac{\partial u_N}{\partial \bm{x}}
\end{equation}
The Jacobian matrix of the dynamics has the following structure:
%  elements are denoted as $A_{ij}$.
\begin{equation}
    \frac{\partial \bm{f}}{\partial \bm{x}} = \begin{bmatrix}
        \bm{0}_{3 \times 3} & I_{3 \times 3} & \bm{0}_{3 \times 1} \\
        A_{vr} & A_{vv} & \bm{a}_{vm} \\
        \bm{0}_{1 \times 3} & \bm{0}_{1 \times 3} & \bm{0}_{1 \times 1}
    \end{bmatrix}
\end{equation}
where $A_{vr}$ and $A_{vv}$ are full, i.e., without any identically null elements, $3 \times 3$ matrices
and $\bm{a}_{vm}$ is a full $3 \times 1$ vector.
% where the expression of matrix $A=\frac{\partial \bm{f}}{\partial \bm{x}}$ is provided in Appendix~B.
The costate equations expand to:
\begin{align}
    \dot{\bm{\lambda}}_r &= -A_{vr}^T \bm{\lambda}_v - \mu_Q \frac{\partial\dot{Q}}{\partial \bm{r}} - 2 \mu_u u_N \frac{\partial u_N}{\partial \bm{r}} \label{eq:dlambda_r} \\
    \dot{\bm{\lambda}}_v &= -\bm{\lambda}_r - A_{vv}^T \bm{\lambda}_v - \mu_Q \frac{\partial\dot{Q}}{\partial \bm{v}} \label{eq:dlambda_v} \\
    \dot{\lambda}_m &= -\bm{a}_{vm} \cdot \bm{\lambda}_v - 2 \mu_u u_N \frac{\partial u_N}{\partial m} \label{eq:dlambda_m}
\end{align}
% \begin{align}
%     \dot{\bm{\lambda}}_r &= -\bm{\lambda}_v - 2 \mu_u u_N \frac{\partial u_N}{\partial \bm{r}} \label{eq:dlambda_r} \\
%     \dot{\bm{\lambda}}_v &= -A_{vr} \bm{\lambda}_r -A_{vv} \bm{\lambda}_v - A_{vm} \lambda_m \label{eq:dlambda_v} \\
%     \dot{\lambda}_m &= - 2 \mu_u u_N \frac{\partial u_N}{\partial m} \label{eq:dlambda_m}
% \end{align}

The transverality conditions at the final boundary are:
\begin{align}
    \bm{\lambda}_r (t_f) &= \mu_1 2 \bm{r}(t_f) + \mu_3 \bm{v}(t_f) + \mu_4 \begin{bmatrix}
        v_y(t_f) & -v_x(t_f) & 0
    \end{bmatrix}^T \label{eq:lambda_r_trans} \\
    \bm{\lambda}_v (t_f) &= \mu_2 2 \bm{v}(t_f) + \mu_3 \bm{r}(t_f) + \mu_4 \begin{bmatrix}
        -y(t_f) & x(t_f) & 0
    \end{bmatrix}^T \label{eq:lambda_v_trans} \\
    \lambda_m (t_f) &= 1 \label{eq:lambda_m_trans}
\end{align}
where $\mu_i$ for $i = 1, \dots, 4$ denote the algebraic multipliers associated with the terminal constraints \eqref{eq:final_radius_nonlinear}--\eqref{eq:final_ainc_circular}.
% A transversality condition useful for the present demonstration is:
% \begin{equation}
%     \lambda_m (t_f) = 1 \label{eq:lambda_m_trans}
% \end{equation}
Finally, since the terminal time $t_f$ is free, the Hamiltonian is null at the final boundary:
\begin{equation}
    H(t_f) = 0 \label{eq:hamiltonian_null}
\end{equation}
\hl{QUESTA E' VERA? O DEVE ESSERE L(tf) = 0? Risposta: L}

Now we show that the constraint \eqref{eq:thrust_direction_cone_con} must be active almost everywhere.
In particular, first we assume that \eqref{eq:thrust_direction_cone_con} is strictly satisfied, i.e., it is not active, and then argue that it is not possible since it generates a contradiction.
%
When Eq.~\eqref{eq:thrust_direction_cone_con} is not active, the complementary condition \eqref{eq:complementary_condition_u} requires that $\mu_u = 0$.
Thus, the KKT condition \eqref{eq:KKT} becomes:
\begin{equation}
    \bm{\lambda}_{v}(t) = \bm{0} \label{eq:lambda_v_null}
\end{equation}
If the transverality condition \eqref{eq:lambda_v_trans} is dot multiplied by $\bm{r}(t_f)$ and $\bm{v}(t_f)$, according to Eqs.~\eqref{eq:final_radius_nonlinear}, \eqref{eq:final_velocity_nonlinear}, and \eqref{eq:final_ainc_circular} we obtain:
\begin{align}
    0 &= \mu_3 a_{\text{des}}^2 \label{eq:mu3_null} \\
    0 &= \mu_2 2 (\mu / a_{\text{des}}) + \mu_4 h_{z, \text{des}} \label{eq:lambda_v_trans_dot_v} 
\end{align}
Eq.~\eqref{eq:mu3_null} implies that $\mu_3 = 0$.
Likewise, the cross product of Eq.~\eqref{eq:lambda_v_trans} by 
% $\bm{r}$ and 
$\bm{v}(t_f)$ produces:
\begin{equation}
    % \bm{0} &= \mu_2 2 \bm{v}(t_f) + \mu_3 \bm{r}(t_f) + \mu_4 \begin{bmatrix}
    %     -y(t_f) & x(t_f) & 0
    % \end{bmatrix}^T \label{eq:lambda_v_trans} \\
    \bm{0} = \mu_4 \begin{bmatrix}
        x(t_f) v_z(t_f) & y(t_f) v_z(t_f) & -x(t_f) v_x(t_f) -y(t_f) v_y(t_f)
    \end{bmatrix}^T \label{eq:lambda_v_trans_cross_v}
\end{equation}
which implies $\mu_4 = 0$ and, thus, $\mu_2 = 0$. 
Substituting $\mu_3$ and $\mu_4$, Eq.~\eqref{eq:lambda_r_trans} reduces to:
\begin{equation}
    \bm{\lambda}_r(t_f) = \mu_1 2 \bm{r}(t_f) \label{eq:lambda_r_parallel_to_r}
\end{equation}
Replacing Eqs.~\eqref{eq:lambda_v_null} and \eqref{eq:lambda_r_parallel_to_r} in Eq.~\eqref{eq:hamiltonian_null} results in:
\begin{equation}
    \mu_1 2 \bm{r}(t_f) \cdot \bm{v}(t_f) + \lambda_m(t_f) (-\dot{m}_e(t_f)) = 0 \label{eq:hamiltonian_null_explicit}
\end{equation}
Due to Eq.~\eqref{eq:final_radial_velocity}, Eq.~\eqref{eq:hamiltonian_null_explicit} requires:
\begin{equation}
    \lambda_m (t_f) = 0 \label{eq:lambda_m_null}
\end{equation}
However, this violates Eq.~\eqref{eq:lambda_m_trans}, thus generating a contradiction.
This contradiction proves that the optimal solution of $\mathcal{P}_R$ must satisfy Eq.~\eqref{eq:thrust_direction_cone_con} with the equality sign. \qed

% % For the purpose of the demonstration, we also suppose that the heat flux constraint is inactive a.e., as stated in Assumption~\ref{assumption:hf}.
% % Thus, according to Eq.~\eqref{eq:complementary_condition_Q}:
% % \begin{equation}
% %     \mu_Q = 0 \label{eq:mu_Q_null}
% % \end{equation}
% Replacing \eqref{eq:lambda_v_null}, \eqref{eq:mu_Q_null}, and $\mu_u = 0$ in the costate equations \eqref{eq:dlambda_r}--\eqref{eq:dlambda_m} leads to:
% \begin{align}
%     \bm{\lambda}_r(t) &= \bm{0} \label{eq:lambda_r_null} \\
%     \dot{\lambda}_m &= 0 \label{eq:lambda_m_const}
% \end{align}
% Because of Eqs.~\eqref{eq:lambda_v_null} and \eqref{eq:lambda_r_null}, the Hamiltonian condition \eqref{eq:hamiltonian_null} requires:
% \begin{equation}
%     \lambda_m (t_f) = 0 \label{eq:lambda_m_null}
% \end{equation}
% However, this violates Eq.~\eqref{eq:lambda_m_trans}, thus generating a contradiction.
% This contradiction proves that the optimal solution of $\mathcal{P}_R$ must satisfy Eq.~\eqref{eq:thrust_direction_cone_con} with the equality sign. \qed

% Eq.~\eqref{eq:lambda_m_trans} combined with Eq.~\eqref{eq:dlambda_m_new} results in:
% \begin{equation}
%     \lambda_m(t) = 1 \label{eq:lambda_m_constant}
% \end{equation}
% Finally, replacing Eq.~\eqref{eq:lambda_m_constant} in Eq.~\eqref{eq:dlambda_v_new} provides an assigned law of $\bm{\lambda}_r$:
% \begin{equation}
%     \bm{\lambda}_r(t) = - A_{vr}^{-1} A_{vm} \label{eq:lambda_r_time_law}
% \end{equation}
% Since Eq.~\eqref{eq:lambda_r_time_law} is a non-constant time law, 

